On Huang and Wong's Algorithm for Generalized Binary Split Trees

Huang and Wong [1984] proposed a polynomial-time dynamic-programming algorithm for computing optimal generalized binary split trees. We show that their algorithm is incorrect. Thus, it remains open whether such trees can be computed in polynomial time. Spuler [1994] proposed modifying Huang and Wong's algorithm to obtain an algorithm for a different problem: computing optimal two-way-comparison search trees. We show that the dynamic program underlying Spuler's algorithm is not valid, in that it does not satisfy the necessary optimal-substructure property and its proposed recurrence relation is incorrect. It remains unknown whether the algorithm is guaranteed to compute a correct overall solution.

==> CODE_huang1984.tex <==
#!/usr/bin/env python3.6
from collections import namedtuple
from functools import lru_cache

memoize = lru_cache(maxsize=None)
Tree = namedtuple('Tree', 'cost weight holes')

def size(i, j, h):
    return j - i + 1 - h

def huang1984(weights):
    '''Returns cost as computed by Huang and Wong's GBSPLIT algorithm (1984).'''

    wts = [weights[k] for k in sorted(weights.keys())]

    @memoize
    def tree(i, j, h):
        '''Returns tree for opt([i,j], h)'''

        if size(i, j, h) == 0:
            return Tree(cost=0, weight=0, holes=frozenset(range(i, j+1)))

        def candidate(k, h_l, h_r):
            left = tree(i, k-1, h_l)
            right = tree(k, j, h_r)
            holes = left.holes | right.holes
            eq_key = min(holes, key=lambda k: wts[k])
            weight = left.weight + right.weight + wts[eq_key]
            return Tree(cost=weight + left.cost + right.cost,
                        weight=weight,
                        holes=holes - {eq_key})

        return min(candidate(k, h_l, h-h_l+1)
                   for k in range(i, j+2)
                   for h_l in range(h+2)
                   if size(i, k-1, h_l) >= 0 and size(k, j, h-h_l+1) >= 0)

    return tree(0, len(weights)-1, 0).cost

# The instance (K, p) from the proof of Theorem 1:
weights = dict(B4=20,
               A3=20, V3=20,
               A2=20, F2=20, T2=20, X2=20,
               A1=20, D1=22, F1=20, Q1=20, S1=20, U1=20, W1=20, Y1=20,
               B0=10, C0= 5, D0=10, E0=10, N0=10, P0=10, Q0=10, R0=10,
               S0=10, T0=10, U0=10, V0=10, W0=10, X0=10, Y0=10, Z0=10)

assert huang1984(weights) == 1763

# Increasing a weight _lowers_ the cost computed by the algorithm.
weights['D1'] += 0.99
assert huang1984(weights) < 1763


==> CODE_spuler1994.tex <==
#!/usr/bin/env python3.6
from collections import namedtuple
from functools import lru_cache

memoize = lru_cache(maxsize=None)
Tree = namedtuple('Tree', 'cost weight holes')

def size(i, j, h):
    return j - i + 1 - h

def spuler1994(wts, n_holes):
    '''Returns cost as computed by Spuler's 2WCST algorithm (1994)'''

    @memoize
    def tree(i, j, h):
        '''Returns tree for opt([i, j], h).'''

        interval = frozenset(range(i, j+1))

        if size(i, j, h) == 1:
            k = min(interval, key=lambda k: wts[k])
            return Tree(cost=0, weight=wts[k], holes=interval - {k})

        def equality_candidate():
            right = tree(i, j, h+1)
            eq_key = min(right.holes, key=lambda k: wts[k])
            return Tree(cost=wts[eq_key] + right.weight + right.cost,
                        weight=wts[eq_key] + right.weight,
                        holes=right.holes - {eq_key})

        def less_than_candidate(k, h_l, h_r):
            left, right = tree(i, k-1, h_l), tree(k, j, h_r)
            return Tree(cost=left.weight + right.weight + left.cost + right.cost,
                        weight=left.weight + right.weight,
                        holes=left.holes | right.holes)

        return min(equality_candidate(),
                   min(less_than_candidate(k, h_l, h-h_l)
                       for k in interval
                       for h_l in range(h+1)
                       if size(i, k-1, h_l) >= 1 and size(k, j, h-h_l) >= 1))

    return tree(0, len(wts)-1, n_holes).cost

# The instance (K, p) and subproblem (I_15, 2) from the proof of Theorem 2:
weights1 = [7, 5, 0, 5, 0, 5, 0, 5, 0, 5, 0, 5, 0, 5, 7]
assert spuler1994(weights1, 2) == 116

# Increasing some weights _lowers_ the cost computed by the algorithm:
weights2 = [9, 5, 0, 5, 0, 5, 0, 5, 0, 5, 0, 5, 0, 5, 9]
assert spuler1994(weights2, 2) == 115

